Batch 1: Definition of several Weather & Climate Dwarfs

This document is one of the deliverable reports created for the ESCAPE project. ESCAPE stands for Energy-efficient Scalable Algorithms for Weather Prediction at Exascale. The project develops world-class, extreme-scale computing capabilities for European operational numerical weather prediction and future climate models. This is done by identifying weather & climate dwarfs which are key patterns in terms of computation and communication (in the spirit of the Berkeley dwarfs). These dwarfs are then optimised for different hardware architectures (single and multi-node) and alternative algorithms are explored. Performance portability is addressed through the use of domain specific languages. This deliverable contains the description of the characteristics of the weather & climate dwarfs that form key functional components of prediction models in terms of the science that they encapsulate and in terms of computational cost they impose on the forecast production. The ESCAPE work flow between work packages centres on these dwarfs and hence their selection, their performance assessment, code adaptation and optimization is crucial for the success of the project. At this stage of ESCAPE, a selection of established and new dwarfs has been made, their documentation been compiled and the software been made available on the software exchange platform. The selection of dwarfs will be extended throughout the course of the project (see Deliverable D1.2). The current selection includes the spectral transforms, the cloud microphysics scheme, two and three-dimensional elliptic solvers, a bi-Fourier spectral transform, an interpolation needed for the semi-Lagrangian advection scheme and a first version of the semi-Lagrangian advection scheme itself. This deliverable includes their scientific description and the guidance for installation, execution and testing.

==> VERSION.tex <==
0.1.0

==> dwarf7.tex <==



\subsubsection{Scope}
\textit{Bespoke scalable, preconditioned non-symmetric solvers} 
are one of the key areas of investigation in terms of Weather 
\& Climate dwarfs.
These arise in large time-step semi-implicit problems within 
compressible or sound-proof atmospheric models.
These solvers can be self-adaptive and may provide robust 
solution procedures for NWP applications. However, their 
scalability properties and effective preconditioning strategies 
must be explored.

Specifically, such solvers are suitable to be adopted in 
conjunction with compact-stencil schemes, such as the finite 
volume method, that are an attractive option for next generation 
HPC facilities given their reduced communication costs (due to 
their intrinsic data locality).

Dwarf 2 implements a promising candidate, namely the Generalised Conjugate 
Residual (GCR) method. This approach aims to provide a robust 
solution procedure for NWP applications required by this key 
investigation area. In particular, the three-dimensional potential-flow 
problem constitutes an excellent benchmark where to experiment 
with different preconditioners to evaluate its competitiveness, 
especially in terms of number of iterations required to reach 
convergence and scalability.



\subsubsection{Objectives}
The main objectives of this dwarf are to improve the computational 
time per iteration of the GCR algorithm and to reduce the number
of iterations to reach convergence. These two aspects are crucial,
since a consistent reduction of the computational cost might allow 
these methods, in conjunction with finite-volume discretizations,
to become very competitive for NWP applications, given their compact 
nature. This is particularly attractive for next-generation HPC 
infrastructures, while retaining a semi-implicit time discretization 
that allows large time-steps.

The evaluation of this dwarf will iclude:
%
\begin{enumerate}
\item Test the GCR approach on different hardware - especially 
GPUs and Accelerators - in order to identify the best solutions 
in terms of computational time per fixed number of iterations. 
Among the best solutions, it will also be necessary to identify 
the best compromise in terms of energy cost.
\item Test the GCR approach applied to the three-dimensional potential 
flow problem, i.e. \inlsh{fvm3d-potential} with different preconditioners 
in order to reduce the number of iterations to reach convergence.
\end{enumerate}
%



\subsubsection{Definition}
Dwarf 2 implements the solution of linear elliptic equations through 
the GCR method \cite{Eisenstat1983,
Smolarkiewicz1994,Smolarkiewicz2000}. 	
Specifically, we solve the potential flow equations that arise when 
discretizing atmospheric flows using a Finite Volume (FV) approach.

In particular, dwarf 2 is constituted by two sub-dwarfs:
%
\begin{itemize}
\item \inlsh{fvm2d-laplacian}, that solves a two-dimensional elliptic 
problem, namely the Laplacian of a simple Gaussian-type function, and 
\item \inlsh{fvm3d-potential}, that solves a three-dimensional elliptic 
problem, namely a potential flow over a Gaussian-shaped hill. 
\end{itemize}
%
Both problems are formulated in spherical coordinates. 
The two-dimensional problem is a prototype to test the basic capabilities
of the method on a simplified case, and it is intended to act as 
a precursor of the main target: the three-dimensional problem defined 
in \inlsh{fvm3-potential}.
In the following, we first describe the GCR method for a general 
linear elliptic problem and then we briefly outline the 
two-dimensional and three-dimensional problems that are available. 



\paragraph{Generalized Conjugate-Residual approach}
In this section we follow closely appendix A of \cite{Thomas2003Spectral}.
In particular, we can formulate the GCR approach starting from the following 
linear elliptic problem:
%
\begin{equation}
\mathcal{L}(\psi) = \sum_{I=1}^{3}\frac{\partial}{\partial x^{I}}
\bigg(\sum_{J=1}^{3}\text{C}^{IJ}\frac{\partial \psi}{\partial x^{J}} 
+ \text{D}^{I}\bigg) - \text{A}\psi = \text{Q},
\label{doc_dwarf7:eq:linear-elliptic}
\end{equation}
%
where A, C$^{IJ}$, D$^{I}$, Q are variable coefficients and for which either 
periodic, Dirichlet or Neumann boundary conditions can be applied.
The discrete representation of a field is denoted by the subscript 
$i$ such that the discrete linear operator is represented by $\mathcal{L}_{i}$
while the inner product by $\langle\xi\,\zeta\rangle = \sum_{i}\xi_{i}\zeta_{i}$.

The GCR approach is formulated in terms of a preconditioner, denoted 
by $\mathcal{P}$, that is a linear operator that approximates $\mathcal{L}$ 
but that is easier to invert. This dwarf is intended to explore just 
left preconditioning strategies. These lead Eq.~\ref{doc_dwarf7:eq:linear-elliptic} 
to be substituted by the auxiliary problem $\mathcal{P}^{-1}[\mathcal{L}(\psi) 
- \text{Q}] = 0$. 

The GCR method presented in \cite{Eisenstat1983}, can then be obtained
through variational arguments (see for instance \cite{Smolarkiewicz1994,
Smolarkiewicz2000}). More specifically, the original problem, 
Eq.~\ref{doc_dwarf7:eq:linear-elliptic}, is augmented by the following $k$th-order 
damped oscillation equation:
%
\begin{equation}
\frac{\partial^{k}\mathcal{P}(\psi)}{\partial\tau^{k}} 
+ \frac{1}{\text{T}_{k-1}(\tau)}\frac{\partial^{k-1}\mathcal{P}(\psi)}{\partial\tau^{k-1}} 
+ \dots + \frac{1}{\text{T}_{1}(\tau)}\frac{\partial\mathcal{P}(\psi)}{\partial\tau} 
= \mathcal{L}(\psi) - \text{Q},
\label{doc_dwarf7:eq:damped}
\end{equation}
%
that is discretized in pseudo-time $\tau$.
This forms the affine discrete equation for the progression of the 
residual errors $r$. The final step is to identify the optimal parameters 
T$_{1}$, ..., T$_{k-1}$ and integration increment $\delta\tau$ that makes sure that 
the minimization of the residual errors in the norm defined by the inner 
product $\langle r\,r \rangle$ is successful.
The steps described leads to the GCR algorithm reported 
in algorithm~\ref{doc_dwarf7:alg:GCR}.
%
\begin{algorithm}[h!]
For any initial guess $\psi_{i}^{0}$, \textbf{set}\\
$r_{i}^{0} = \mathcal{L}(\psi^{0}) - \text{Q}_{i}$\\
$p_{i}^{0} = \mathcal{P}^{-1}(r^{0})$, \textbf{then}:\\[0.5em]
\SetAlgoLined
\For{n = 1,2,...,until convergence}{
 \For{$\nu$ = 0,1,...,k-1}{
   \vspace{.4cm}
   % -------------------------------------------------------------
   $\displaystyle 
   \beta = -\frac{\langle r^{\nu}\,\mathcal{L}(p^{\nu})\rangle}{
   \mathcal{L}(p^{\nu})\,\mathcal{L}(p^{\nu})}$\\[1em]
   % -------------------------------------------------------------
   $\displaystyle 
   \psi^{\nu+1}_{i} = \psi^{\nu}_{i} + \beta\,p^{\nu}_{i}$\\[1em]
   % -------------------------------------------------------------
   $\displaystyle
   r^{\nu+1}_{i} = r^{\nu}_{i} + \beta\mathcal{L}_{i}(p^{\nu})$\\[1em]
   % -------------------------------------------------------------
   \textbf{if} $\Vert r^{\nu+1}\Vert \leq \epsilon$ \textbf{then} exit\\[1em]
   % -------------------------------------------------------------
   $\displaystyle  
   e_{i} = \mathcal{P}^{-1}_{i}(r^{\nu+1})$\\[1em]
   % -------------------------------------------------------------
   $\displaystyle
   \mathcal{L}_{i}(e) = \bigg[\sum_{I=1}^{3}\frac{\partial}{\partial x^{I}}
   \bigg(\sum_{J=1}^{3}\text{C}^{IJ}\frac{\partial e}{\partial x^{J}} + 
   \text{D}^{I}\,e\bigg) - A\,e\bigg]_{i}$\\[1em]
   % -------------------------------------------------------------
   $\displaystyle
   \textbf{for}\; \ell=0,...,\nu\;\;\;\alpha_{\ell} = 
   -\frac{\langle \mathcal{L}(e)\,\mathcal{L}(p^{\ell})\rangle}{\langle
   \mathcal{L}(p^{\ell})\,\mathcal{L}(p^{\ell})\rangle}$\\[1em]
   % -------------------------------------------------------------
   $\displaystyle
   p^{\nu+1}_{i} = e_{i} +     
   \sum_{\ell=0}^{\nu}\alpha_{\ell}\,p^{\ell}_{i}$\\[1em]
   % -------------------------------------------------------------
   $\displaystyle
   \mathcal{L}_{i}(p^{\nu+1}) = \mathcal{L}_{i}(e) + 
   \sum_{\ell=0}^{\nu}\alpha_{\ell}\,\mathcal{L}^{\ell}_{i}(p^{\ell})$
   % -------------------------------------------------------------
 }
 reset [$\psi$, $r$, $p$, $\mathcal{L}$]$_{i}^{k}$ 
 to [$\psi$, $r$, $p$, $\mathcal{L}$]$_{i}^{0}$
}
\caption{Generalized Conjugate Residual (GCR) method}
\label{doc_dwarf7:alg:GCR}
\end{algorithm}




\paragraph{Two-dimensional Laplacian problem}
The two-dimensional version of dwarf 2 is constituted 
by the following Laplacian problem on the sphere:
%
\begin{equation}
\nabla^{2}\psi(x,y) = \mathcal{R},
\label{doc_dwarf7:eq:laplacian}
\end{equation}  
%
where $\mathcal{R}$ is the right-hand side and it consists 
of the Laplacian of $\psi_0$, while $\psi_0$ is a scalar 
function whose initial value is set equal to a Gaussian-shaped 
hill, that is:
%
\begin{align}
s(x,y) = 2\,\sqrt{\cos(y)\,\sin\bigg(\frac{x - x_{c}}{2}\bigg)\,
\sin\bigg(\frac{y - y_{c}}{2}\bigg)} &
& \nonumber \\[1em]
\psi_{0}(x,y) = \left\{
\begin{array}{ll}
\displaystyle \frac{\kappa}{2}\Big[1 
+ \cos\Big(\pi \frac{s}{2\pi/9}\Big)\Big], 
& \forall s < 2\pi/9\\[1em]
0, & \forall s \geq 2\pi/9 .
\end{array}
\right.
\label{doc_dwarf7:eq:2d-initial}
\end{align}  
%
Variables $x$, $y$ denote the coordinates of the longitude and 
latitude, respectively, $x_{c}$, $y_{c}$ denote the centre of 
the hill in the longitude and latitude direction, respectively, 
and $\kappa$ denotes the height of the hill. The numerical 
discretization of Eq.~\ref{doc_dwarf7:eq:laplacian} is achieved by 
a FV method on the sphere, with differentiation across 
the pole following \cite{Smolarkiewicz2016}. The detailed 
set of equations involved in this problem is not reported 
here because it is beyond the scope of this documentation.
However, we provide a concise description of the procedure.
In particular, the solution is computed by calculating 
the Laplacian through a Green-Gauss strategy in spherical 
coordinates. 
The Laplacian calculated in this way is the right-hand side 
$\mathcal{R}$ in Eq.~\ref{doc_dwarf7:eq:laplacian}. This right-hand 
side is then provided as an argument to the GCR routine 
where $\psi_{\text{GCR}}$ is calculated. The result of 
the GCR routine should recover the initial value of $\psi$, 
i.e. Eq.~\ref{doc_dwarf7:eq:2d-initial}.

The error is finally computed by taking the difference between 
the initial value $\psi_{0}$ and its calculated value through 
the GCR algorithm $\psi_{\text{GCR}}$. Note that the GCR routine 
applied to a FV approach is subject to the so-called 
null-spaces. This means that the solution is affected by an arbitrary 
offset which corresponds to the mean value of the difference 
between the initial guess and the GCR-calculated solution:
%
\begin{equation}
\overline{err} = \frac{\sum_{j=1}^{N}|\psi_{0,j} - \psi_{\text{GCR},j}|}{N},
\label{doc_dwarf7:eq:error}
\end{equation}
% 
where $N$ is the total number of solution points, the subscript 
$j$ denotes the $j$-th solution point, $\psi_{0,j}$ is the initial 
values of the function, $\psi_{GCR,j}$ is the value of the function
calculated using the GCR approach and $\bar{err}$ is the mean error 
due to the null-spaces.



\paragraph{Three-dimensional potential-flow problem}
The three-dimensional version of dwarf 2 solves a potential flow 
over a Gaussian-shaped hill. The governing equations of this problem 
may be written as follows:
%
\begin{equation}
\begin{array}{l}
\boldsymbol{v} = \boldsymbol{v}_{e} - \nabla\phi\\[0.5em]
\nabla\cdot(\rho\boldsymbol{v}) = 0
\end{array}
\label{doc_dwarf7:eq:potential}
\end{equation}  
%
where $\boldsymbol{v}_{e}$ is the ambient velocity which can be 
obtained from measurments or prescribed analitically and $\overline{\rho} = 
\overline{\rho}(z)$ is the reference density. In the above problem, 
we seek $\phi$ such that it satisfies the set of equations we aim 
to solve, thus providing a better initial guess for the given problem. 
Equation~\ref{doc_dwarf7:eq:potential} 
is cast in a non-orthogonal terrain-following systems of coordinates, 
$[x,y,z] = [x_{\text{cart}},y_{\text{cart}},H(z_{\text{cart}} - h)/(H - h]$,
with the subscript 'cart' referring to Cartesian coordinates, $H$
to the model depth and $h = h(x_{\text{cart}},y_{\text{cart}})$ 
to the mountain profile. 
The transformation of Eq.~\ref{doc_dwarf7:eq:potential} from the Cartesian 
frame of reference to the terrain-following frame of reference 
involves some metric terms that are fairly standard in atmospheric 
applications.
In particular, we can introduce the following transformation matrix
and Jacobian:
%
\begin{equation}
\begin{array}{l}
\displaystyle \text{G}^{IJ} = \sum_{K=1}^{2}\frac{\partial x^{I}}{\partial x_{\text{cart}}^{K}}
\frac{\partial x^{J}}{\partial x_{\text{cart}}^{K}}\\[0.5em]
\displaystyle \text{J} = \big[det(\text{G}^{IJ})\big]^{1/2},
\end{array}
\label{doc_dwarf7:eq:2d-transformations} 
\end{equation}
%
where the subscript `cart' denotes Cartesian coordinates.
For additional information the interested reader can refer 
to \cite{Smolarkiewicz1994}. 
Using these quantities, the original problem in Eq.~\ref{doc_dwarf7:eq:potential}
becomes:
%
\begin{equation}
\begin{array}{l}
\displaystyle u = u_{e} - \frac{\partial\phi}{\partial x} 
- \text{G}^{13}\frac{\partial\phi}{\partial z}\\[0.75em]
\displaystyle v = v_{e} - \frac{\partial\phi}{\partial y} 
- \text{G}^{23}\frac{\partial\phi}{\partial z}\\[0.75em]
\displaystyle w = w_{e} - \text{J}^{-1}\frac{\partial\phi}{\partial z}\\[0.75em]
\displaystyle \frac{\partial \rho^{*}u}{\partial x} + 
\frac{\partial \rho^{*}v}{\partial y} + 
\frac{\partial\rho^{*}\omega}{\partial z} = 0,
\end{array}
\label{doc_dwarf7:eq:transformed}
\end{equation}
%
where $\rho^{*} = \text{J}\overline{\rho}$ and the contravariant 
velocity $\omega$ is defined as $\omega = \text{J}^{-1}w + \text{G}^{13}u 
+ \text{G}^{23}v$. 

To obtain the associated boundary-value problem, we perform three steps.
We first substitute the $u$, $v$ and $w$ into the contravariant velocity 
$\omega$, we then substitute $u$, $v$ and the just obtained contravariant 
velocity $\omega$ into the last equation in Eq.~\ref{doc_dwarf7:eq:transformed}.
These first two steps lead to the following problem:
%
\begin{equation}
\nabla\cdot\Big(\rho^{*}\mathbf{P}_{f}(\phi,\nabla\phi)\Big),
\label{doc_dwarf7:eq:manipulated}
\end{equation}
%
where the components of the pressure force vector $\mathbf{P}_{f}$
are defined as follows:
%
\begin{equation}
\begin{array}{l}
\displaystyle \mathbf{p}_{f,x} = u\\[0.5em]
\displaystyle \mathbf{p}_{f,y} = v\\[0.5em]
\displaystyle \mathbf{p}_{f,z} = \omega_{e} - 
\text{G}^{13}\frac{\partial\phi}{\partial x} - 
\text{G}^{23}\frac{\partial\phi}{\partial y} - 
\text{G}^{33}\frac{\partial\phi}{\partial z}
\end{array}
\label{doc_dwarf7:eq:transformed}
\end{equation}
%
with $\omega_{e} = \text{J}^{-1}w_{e} + \text{G}^{13}u_{e} + \text{G}^{23}v_{e}$
and $\text{G}^{33} = (\text{G}^{13})^{2} + (\text{G}^{23})^{2} + 1/\text{J}^{2}$.
The third step involves multiplying Eq.~\ref{doc_dwarf7:eq:manipulated} 
by $-1/\rho^{*}$. This finally leads to the following equation:  
%
\begin{equation}
-\frac{1}{\rho^{*}}\nabla\cdot\bigg(\rho^{*}\boldsymbol{P}_{f}
(\phi,\nabla\phi)\bigg) = \frac{1}{\rho^{*}}\nabla\cdot\bigg(
\rho^{*}\big(\boldsymbol{v}^{*} - \boldsymbol{P}_{f}\big)\bigg) 
= 0,
\label{doc_dwarf7:eq:potential}
\end{equation}  
%
that is solved using the GCR algorithm introduced above.
For additional details on this model problem refer to 
\cite{Smolarkiewicz1994}. Note that this is the target 
problem for this dwarf.



\subsubsection{Dwarf usage and testing}
In this section we describe how to download and install 
the dwarf along with all its dependencies, and we show 
how to run it for a simple test case.

Note that dwarf 2 is implemented using \textit{Atlas}, 
the ECMWF software framework that supports flexible 
data-structures for NWP. Currently, the two sub-dwarfs 
are written in Fortran 2003. Extensions to C++ can 
be envisioned if necessary and they can be implemented 
using \textit{Atlas}.



\paragraph{Download and installation}
The first step is to download and install the dwarf along 
with all its dependencies. With this purpose, it is possible 
to use the script provided under the ESCAPE software collaboration 
platform:\\
\url{https://software.ecmwf.int/stash/projects/ESCAPE}.

Here you can find a repository called \inlsh{escape}.
You need to download it. You could first create a 
folder named, for instance, ESCAPE, enter into it 
and subsequently download the repository. Inside the network of ECMWF you can use the following the steps below:
%
\begin{lstlisting}[style=BashStyle]
mkdir ESCAPE
cd ESCAPE/
git clone ssh://git@software.ecmwf.int:7999/escape/escape.git
\end{lstlisting}
%
If you are an external project partner (i.e. not in the network of ECMWF) you need to use https instead of ssh. Once the repository is downloaded into the \inlsh{ESCAPE} folder 
just created, you should find a new folder called \inlsh{escape}. 
The folder contains a sub-folder called \inlsh{bin} that has the 
python/bash script (called \inlsh{escape}) that needs to be 
run for downloading and installing the dwarf and its dependencies. 
To see the various options provided by the script you can type:
%
\begin{lstlisting}[style=BashStyle]
./escape/bin/escape -h
\end{lstlisting}
%
To download the dwarf and its dependencies you need to run 
the following command:
%
\begin{lstlisting}[style=BashStyle]
./escape/bin/escape checkout dwarf2-ellipticsolver --ssh
\end{lstlisting}
% 
Note the option \inlsh{--ssh}. This can be used only internally 
at ECMWF for the moment. If you are an external project partner
you should use the following command instead:
%
\begin{lstlisting}[style=BashStyle]
./escape/bin/escape checkout dwarf2-ellipticsolver --user <username>
\end{lstlisting}
% 
and follow the instructions. 
The commands above automatically check out the \inlsh{develop}
version of the dwarf. If you want to download a specific branch 
of this dwarf, you can do so by typing:
%
\begin{lstlisting}[style=BashStyle]
./escape/bin/escape checkout dwarf2-ellipticsolver --ssh \
--version <branch-name>
\end{lstlisting}
% 
An analogous approach can be used for the \inlsh{-\,-user} 
version of the command. You should now have a folder called 
\inlsh{dwarf2-ellipticsolver}.

In the above command, you can specify several other optional 
parameters. To see all these options and how to use them you 
can type the following command:
%
\begin{lstlisting}[style=BashStyle]
./escape checkout -h
\end{lstlisting}
%

At this stage it is possible to install the dwarf 
and all its dependencies. This can be done in two 
different ways. The first way is to compile and 
install each dependency and the dwarf separately:
%
\begin{lstlisting}[style=BashStyle]
./escape/bin/escape generate_install dwarf2-ellipticsolver
\end{lstlisting}
% 
The command above will generate a script 
called \inlsh{install-dwarf2-ellipticsolver} 
that can be run by typing:
%
\begin{lstlisting}[style=BashStyle]
./install-dwarf2-ellipticsolver
\end{lstlisting}
%
This last step will build and install the dwarf 
along with all its dependencies in the following 
paths:
%
\begin{lstlisting}[style=BashStyle]
dwarf2-ellipticsolver/builds/
dwarf2-ellipticsolver/install/
\end{lstlisting}
%

The second way is to create a bundle that compiles 
and installs all the dependencies together:
%
\begin{lstlisting}[style=BashStyle]
./escape/bin/escape generate_bundle dwarf2-ellipticsolver
\end{lstlisting}
% 
This command will create an infrastructure to avoid
compiling the single third-party libraries individually
when some modifications are applied locally to one of 
them. To complete the compilation and installation process, 
after having run the above command for the bundle, simply 
follow the instructions on the terminal.

In the commands above that generate the installation 
file, you can specify several other optional parameters. 
To see all these options and how to use them you 
can type the following command:
%
\begin{lstlisting}[style=BashStyle]
./escape generate-install -h
./escape generate-bundle -h
\end{lstlisting}
%

\paragraph{Testing}
You should now verify that the dwarf works as expected.
For this purpose, we created a testing framework that
allows us to verify that the main features of the dwarf 
are working correctly.

In particular, for each sub-dwarf we provide various 
regression tests in order to allow the results to be 
consistent when the underlying algorithms are modified, 
and to test additional features or different hardware. 
The regression tests can be found in the folder \inlsh{test} 
that is located in each sub-dwarf folder. 
For each sub-dwarf we also provide scripts running the 
code on different architectures, e.g. the Cray HPC at 
ECMWF, that can be found in the folder \inlsh{run-scripts} 
located in each sub-dwarf folder. 
%
\begin{tipbox}
We encourage partners who are testing different architectures 
to add and/or modify the scripts!
\end{tipbox}
%

To run this verification, you should run the following 
command:
%
\begin{lstlisting}[style=BashStyle]
ctest -j<number-of-tasks>
\end{lstlisting}
%
from inside the \inlsh{builds/dwarf2-ellipticsolver}
folder.
%
\begin{warningbox}
We strongly advise you to verify via ctest that 
the main functionalities of the dwarf are working 
properly any time you apply modifications to the 
code. Updates that do not pass the tests cannot 
be merged. 
In addition, if you add a new feature to the dwarf,
this should be supported by a test if the existing
testing framework is not already able to verify its
functionality.
\end{warningbox}
%
For instructions on how to run the executables 
see the next section.



\subsubsection{Run the Dwarf}
If you want to run the dwarf in your local machine, 
you could do so by using the executable files inside 
%
\begin{lstlisting}[style=BashStyle] 
dwarf2-ellipticsolver/install/dwarf2-ellipticsolver/bin/
\end{lstlisting}
%
In particular, the executables need the specification 
of a configuration file. This dwarf is constituted 
by two different sub-dwarfs, a two-dimensional and 
a three-dimensional version. The configuration files, 
one for each version, can be found at
%
\begin{lstlisting}[style=BashStyle] 
dwarf2-ellipticsolver/sources/dwarf2-ellipticsolver/config-files/
\end{lstlisting}
%
These are \inlsh{dwarf2-fvm2d-O32.json} and \inlsh{dwarf2-fvm3d-O32.json}. 
Each of them specify some parameters needed by each sub-dwarf. 
In the next two subsections we specify how to run each sub-dwarf 
and explain the parameters inside the \inlsh{.json} files.


\paragraph{Run the two-dimensional problem: dwarf2-fvm2d}
The two-dimensional problem is constituted by a Laplacian 
operator. 
To run it you should copy the \inlsh{dwarf2-fvm2d-O32.json} 
file in the folder where you want to run the simulation 
(or alternatively specify its path on the command line). 
The executable can then be run as follows:
%
\begin{lstlisting}[style=BashStyle] 
dwarf2-ellipticsolver/install/dwarf2-ellipticsolver/bin/dwarf2-fvm2d \
--config dwarf2-fvm2d-O32.json
\end{lstlisting}
%
where, if the \inlsh{.json} file is not in the current directory, 
you can specify its path after \inlsh{-\,-config}.

If you instead want to run the dwarf on an HPC machine 
available to the ESCAPE partners, you can automatically 
generate the job submission script with the \inlsh{escape} 
file. 

More specifically, if you run the following command:
%
\begin{lstlisting}[style=BashStyle]
./escape generate-run -c \
dwarf2-ellipticsolver/install/dwarf2-ellipticsolver/bin/dwarf2-fvm2d \
--config dwarf2-fvm2d-O32.json
\end{lstlisting}
% 
This allows the code to generate the submission script      
for the given HPC machine you are targeting without submitting
the actual job. The command above will in fact simply generate
an \inlsh{escape.job} file in the current folder. This can
successively be submitted via \inlsh{qsub} on the HPC machine
you want to run the simulation on.

In the above command you can specify several other optional 
parameters, such as wall-time, number of tasks, number of 
threads, etc. To see all these options and how to set them 
up you can type the following command:
%
\begin{lstlisting}[style=BashStyle]
./escape generate-run -h
\end{lstlisting}
%


 
\paragraph{Run the three-dimensional problem: dwarf2-fvm3d}
The three-dimensional version of dwarf 2, implements a potential 
flow problem over an idealised hill. To run it you should copy 
the \inlsh{dwarf2-fvm3d-O32.json} file in the folder where you 
want to run the simulation (or alternatively specify its path 
on the command line). The executable can then be run as follows:
%
\begin{lstlisting}[style=BashStyle] 
dwarf2-ellipticsolver/install/dwarf2-ellipticsolver/bin/dwarf2-fvm2d \
--config dwarf2-fvm3d-O32.json
\end{lstlisting}
%
where, if the \inlsh{.json} file is not in the current directory, 
you can specify its path after \inlsh{-\,-config}.

If you instead want to run the dwarf on an HPC machine 
available to the ESCAPE partners, you can automatically 
generate the job submission script with the \inlsh{escape} 
file. More specifically, if you run the following command:
%
\begin{lstlisting}[style=BashStyle]
./escape generate-run -c \
dwarf2-ellipticsolver/install/dwarf2-ellipticsolver/bin/dwarf2-fvm3d \
--config dwarf2-fvm3d-O32.json
\end{lstlisting}
% 
This allows the code to generate the submission script 
for the given HPC machine you are targeting without submitting 
the actual job. The command above will in fact simply generate 
an \inlsh{escape.job} file in the current folder. This can
successively be submitted via \inlsh{qsub} on the HPC machine 
you want to run the simulation on.

In the above command you can specify several other optional 
parameters, such as wall-time, number of tasks, number of 
threads, etc. To see all these options and how to set them 
up you can type the following command:
%
\begin{lstlisting}[style=BashStyle]
./escape generate-run -h
\end{lstlisting}
%


\subsubsection{Integration}
This dwarf explores the solution of a linear elliptic operator
in spherical coordinates and that arises in the context of mesh-based 
discretizations (such as the finite volume method). 
In particular, this dwarf can be integrated in a global Weather 
\& Climate model involving a semi-implicit time-stepping scheme 
and a mesh-based spatial discretization. This, for instance, 
arises in the solution of the horizontal part of an NWP model.

So, the key aspects for this dwarf to be integrated within a 
Weather \& Climate model are:
%
\begin{itemize}
\item Solution of the horizontal part of a three-dimensional NWP model.
\item Mesh-based discretization (e.g. finite-volume or finite-element 
methods);
\item Semi-implicit discretization in time;
\end{itemize}
%
If these three aspects are present in the NWP model, this dwarf can 
be integrated to solve the horizontal Laplacian of the model in a semi-implicit
and mesh-based manner.







